Puddles: Application-Independent Recovery and Location-Independent Data for Persistent Memory

In this paper, we argue that current work has failed to provide a comprehensive and maintainable in-memory representation for persistent memory. PM data should be easily mappable into a process address space, shareable across processes, shippable between machines, consistent after a crash, and accessible to legacy code with fast, efficient pointers as first-class abstractions. While existing systems have provided niceties like mmap()-based load/store access, they have not been able to support all these necessary properties due to conflicting requirements. We propose Puddles, a new persistent memory abstraction, to solve these problems. Puddles provide application-independent recovery after a power outage; they make recovery from a system failure a system-level property of the stored data rather than the responsibility of the programs that access it. Puddles use native pointers, so they are compatible with existing code. Finally, Puddles implement support for sharing and shipping of PM data between processes and systems without expensive serialization and deserialization. Compared to existing systems, Puddles are at least as fast as and up to 1.34$\times$ faster than PMDK while being competitive with other PM libraries across YCSB workloads. Moreover, to demonstrate Puddles' ability to relocate data, we showcase a sensor network data-aggregation workload that results in a 4.7$\times$ speedup over PMDK.

==> preamble.tex <==
\RequirePackage[normalem]{ulem}
\RequirePackage{color}\definecolor{RED}{rgb}{1,0,0}\definecolor{BLUE}{rgb}{0,0,1}
\providecommand{\DIFadd}[1]{{\color{blue}#1}}
\providecommand{\DIFdel}[1]{{\color{red}\sout{#1}}}   

